Multiband GPI Imaging of the HR 4796A Debris Disk

We have obtained Gemini Planet Imager (GPI) J-, H-, K1-, and K2-Spec observations of the iconic debris ring around the young, main-sequence star HR 4796A. We applied several point-spread function (PSF) subtraction techniques to the observations (Mask-and-Interpolate, RDI-NMF, RDI-KLIP, and ADI-KLIP) to measure the geometric parameters and the scattering phase function for the disk. To understand the systematic errors associated with PSF subtraction, we also forward-modeled the observations using a Markov Chain Monte Carlo framework and a simple model for the disk. We found that measurements of the disk geometric parameters were robust, with all of our analyses yielding consistent results; however, measurements of the scattering phase function were challenging to reconstruct from PSF-subtracted images, despite extensive testing. As a result, we estimated the scattering phase function using disk modeling. We searched for a dependence of the scattering phase function with respect to the GPI filters but found none. We compared the H-band scattering phase function with that measured by Hubble Space Telescope STIS at visual wavelengths and discovered a blue color at small scattering angles and a red color at large scattering angles, consistent with predictions and laboratory measurements of large grains. Finally, we successfully modeled the SPHERE H2 HR 4796A scattered phase function using a distribution of hollow spheres composed of silicates, carbon, and metallic iron.

==> GPI HR 4796A Total Intensity Phase Function arxive version/table1.tex <==
\ProvidesFile{table1.tex}

\begin{deluxetable*}{llccccccc}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Observations\label{tab:observations}}
\tablewidth{0pt}
\tablehead{
    \colhead{Target} &
    \colhead{UT Date} &
    \colhead{Program} &
    \colhead{Obs. Mode$^{a}$} &
    \colhead{Int.Time} &
    \colhead{No. of} &
    \colhead{Airmass} &
    \colhead{Seeing} &
    \colhead{Field Rot.$^{b}$} \\
    \omit &
    \omit &
    \omit &
    \omit &
    \colhead{(s)} &
    \colhead{Exps.} &
    \omit &
    \colhead{($\arcsec$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{10}
\startdata
HR 4796A & 2016 Mar 23 & GS-2016A-LP-6 & J-Spec$^{c}$ & 29.1 & 59 &  1.02-1.04 & 0.4-0.7 & 48.8 \\ %\hline
HR 4796A & 2016 Mar 18 & GS-2016A-Q-500 & H-Spec & 59.6 & 37 & 1.01-1.02 & 0.5 & 52.7 \\
HR 4796A & 2014 Mar 25 & GS-ENG-GPI-COM & K1-Spec & 59.6 & 20 & 1.01-1.02 & 0.3 & 15.1, 12.6 \\ 
HR 4796A & 2015 Apr 2 & GS-2015A-Q-27 & K1-Spec & 88.7 & 47 & 1.13-1.24, 1.11-1.21 & 0.55 & 8.0, 8.4 \\
HR 4796A & 2015 Apr 3 & GS-2015A-Q-27 & K1-Spec & 88.7 & 46 & 1.01-1.09 & 0.55 & 78.5 \\
HR 4796A & 2015 Apr 3 & GS-2015A-Q-27 & K2-Spec & 88.7 & 23 & 1.02-1.04 & 0.55 & 33.8 \\
%HR 2562 & 2016 Mar 18 & GS-2016A-Q-500 & K2-Spec & 59.6 & 47 & 1.15-1.17 & 0.8 & 25.7 \\
\enddata
\tablecomments{$^{a}$ GPI instrument mode corresponding to choice of filter plus corresponding focal plane and Lyot plane masks and apodizer.\\ $^{b}$ Change in parallactic angle over the course of the observation sequence.\\ $^{c}$ Observation made with nonstandard apodizer (APOD$\_$H$\_$G6205).}
\end{deluxetable*}
\endinput


==> GPI HR 4796A Total Intensity Phase Function arxive version/table2.tex <==
\ProvidesFile{table2.tex}

\begin{deluxetable*}{rcccccccccr}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Debris Ring Analyzer Geometric Parameters (Sky-Plane and Disk-Plane)\label{tab:geoparam}} 
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$a'$} &
    \colhead{$e'$} &
    \colhead{$PA'$} &
    \colhead{$\Delta$R.A.$'$} &
    \colhead{$\Delta$Dec.$'$} &
    \colhead{$a$} &
    \colhead{$e$} &
    \colhead{$i$} &
    \colhead{$\omega$} &
    \colhead{$\Omega$} \\
    \omit &
    \colhead{($mas$)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{(mas)} &
    \colhead{(mas)} &
    \colhead{($mas$)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{11}
\startdata
\cutinhead{Mask-and-Interpolate}
   $J$ 20160323 & 1053$\pm$6  & 0.970$\pm$0.001 & 26.2$\pm$0.5   & 6$\pm$4 & -15$\pm$7 & 1053$\pm$6  & 0.02$\pm$0.01 & 75.9$\pm$0.1 & -22$\pm$56 & 26.2$\pm$0.5 \\
   $H$ 20160318 & 1063$\pm$16  &  0.970$\pm$0.002  & 26.5$\pm$0.4 & 0$\pm$8 &  -6$\pm$11 & 1063$\pm$16  &  0.01$\pm$0.02  & 76.5$\pm$0.5 & -61$\pm$180  & 26.5$\pm$0.4 \\
$K_{1}$ 20140325 & 1079$\pm$27  & 0.970$\pm$0.002 & 26.5$\pm$0.4  & 4$\pm$10 & -17$\pm$19 & 1079$\pm$28  & 0.02$\pm$0.02 & 77.0$\pm$0.6 & -44$\pm$62 & 26.5$\pm$0.4 \\ 
$K_{1}$ 20150402 & 1060$\pm$12  & 0.972$\pm$0.002 & 26.6$\pm$0.4  & -1$\pm$6 & -20$\pm$10 & 1061$\pm$12  & 0.04$\pm$0.02 & 76.4$\pm$0.5 & -67$\pm$19 & 26.6$\pm$0.4 \\
$K_{1}$ 20150403 & 1066$\pm$22  & 0.973$\pm$0.002 & 26.5$\pm$0.4  & 8$\pm$8 & -19$\pm$12 & 1066$\pm$22  & 0.02$\pm$0.01 & 76.5$\pm$0.6 & -14$\pm$46 & 26.5$\pm$0.4 \\
$K_{2}$ 20150403 & 1075$\pm$30 &  0.973$\pm$0.003  & 26.5$\pm$0.5 & -6$\pm$9 &  -13$\pm$16 & 1076$\pm$30 & 0.05$\pm$0.02 & 76.7$\pm$0.7 & -79$\pm$22 & 26.5$\pm$0.5 \\
\cutinhead{RDI-NMF}
   $H$ 20160318 & 1069$\pm$18  &  0.970$\pm$0.002  & 26.5$\pm$0.5 & -1$\pm$9 & -14$\pm$14 & 1070$\pm$18  &  0.03$\pm$0.02  & 76.5$\pm$0.5 & -68$\pm$50 & 26.5$\pm$0.5 \\
\cutinhead{RDI-KLIP}
   $H$ 20160318 & 1063$\pm$15  &  0.972$\pm$0.001  & 26.5$\pm$0.4 & 0$\pm$7 & -15$\pm$11 & 1063$\pm$15  &  0.03$\pm$0.01  & 76.3$\pm$0.4 & -65$\pm$30  & 26.5$\pm$0.4 \\
\cutinhead{ADI-KLIP}
   $J$ 20160323 & 1069$\pm$14 & 0.972$\pm$0.002 & 26.5$\pm$0.5 & 2$\pm$7 & -18$\pm$11 & 1069$\pm$14 & 0.03$\pm$0.02 & 76.5$\pm$0.5 & -58$\pm$43 & 26.5$\pm$0.5 \\
   $H$ 20160318 & 1069$\pm$15 & 0.972$\pm$0.002 & 26.5$\pm$0.4 & 0$\pm$7 & -15$\pm$10 & 1069$\pm$15 & 0.03$\pm$0.02 & 76.5$\pm$0.4 & -65$\pm$35 & 26.5$\pm$0.4 \\
$K_{1}$ 20140325 & 1070$\pm$22 & 0.972$\pm$0.002 & 26.4$\pm$0.5 & 1$\pm$9 & -21$\pm$16 & 1070$\pm$22 & 0.04$\pm$0.02 & 76.4$\pm$0.5 & -61$\pm$23 & 26.4$\pm$0.5 \\ 
$K_{1}$ 20150402 & 1077$\pm$16 & 0.973$\pm$0.002 & 26.4$\pm$0.4 & -2$\pm$8 & -21$\pm$13 & 1078$\pm$16 & 0.05$\pm$0.02 & 76.7$\pm$0.5 &  -69$\pm$23 & 26.4$\pm$0.4 \\
$K_{1}$ 20150403 & 1069$\pm$13  & 0.972$\pm$0.002 & 26.4$\pm$0.5  & 1$\pm$7 & -24$\pm$11 & 1069$\pm$13  & 0.04$\pm$0.02 & 76.4$\pm$0.4 & -62$\pm$21 & 26.4$\pm$0.5 \\
$K_{2}$ 20150403 & 1074$\pm$18 &  0.973$\pm$0.002  & 26.5$\pm$0.5 & 0$\pm$8 &  -23$\pm$13 & 1076$\pm$18 & 0.05$\pm$0.02 & 76.6$\pm$0.5 & -65$\pm$24 & 26.5$\pm$0.5 \\
\enddata
\tablecomments{The uncertainties listed in this table are the statistical uncertainties from our fits and do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14}}
%\tablecomments{$^{b}$Change in parallactic angle over the course of the observation sequence}
\end{deluxetable*}

\endinput


==> GPI HR 4796A Total Intensity Phase Function arxive version/table3.tex <==
\ProvidesFile{table3.tex}


\begin{deluxetable*}{lccccc}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Disk Fitting Geometry Parameters (Disk Plane)\label{tab:mcmc_geometry_param}}
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$R_1$} &
    \colhead{$e$} &
    \colhead{$i$} &
    \colhead{$\omega$} &
    \colhead{$\Omega$} \\
    \omit &
    \colhead{(mas)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{11}
\startdata
GPI $J$ 20160323 & 1038$\pm$5 & 0.023$\pm$0.004 & 76.9$\pm$0.1 & -28$^{+15}_{-13}$ & 26.8$\pm$0.1 \\
SPHERE $H_2^{*}$ & 1032 $\pm$1 & 0.047$\pm$0.002 & 76.77$\pm$0.03 & -65$\pm$1 & 26.94$\pm$0.04 \\ 
GPI $H$ 20160318 & 1032$\pm$2 & 0.028$\pm$0.003 & 76.81$\pm$0.07 & -64$\pm$4 & 26.7$\pm$0.1\\
GPI $K_{1}$ 20150403 & 1031$\pm$4 & 0.035$^{+0.003}_{-0.002}$ & 76.47$^{+0.07}_{-0.08}$ & -46$\pm$4 & 26.6$\pm$0.6\\
GPI $K_{2}$ 20150403 & 1036$^{+6}_{-7}$ & 0.024$\pm$0.004 & 76.6$\pm$0.1 & -42$^{+12}_{-11}$ & 26.5$\pm$0.1\\
\enddata
\tablenotetext{*}{Derived from a reanalysis of the data as presented in this manuscript and not from \citetalias{milli17}}
\tablecomments{The uncertainties listed in this table are derived from the 16\%, 50\%, and 84\% percentiles of the marginalized posterior distribution for each parameter and for each dataset. They do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14} and 0.08$\arcdeg$ for SPHERE/IRDIS \citep{maire16}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14} and 0.25 pixels (or 3 mas) for SPHERE/IRDIS (\citetalias{milli17}).}
\end{deluxetable*}
\endinput



% \begin{deluxetable*}{rcccccccccc}
% %\tabletypesize{\scriptsize}
% %\rotate
% \tablecaption{Disk Fitting Geometry Parameters\label{tab:mcmcparam}}
% \tablewidth{0pt}
% \tablehead{
%     \omit &
%     \colhead{$R_1'$} &
%     \colhead{$R_2'$} &
%     \colhead{$PA'$} &
%     \colhead{$\Delta$R.A.$'$} &
%     \colhead{$\Delta$Dec.$'$} &
%     \colhead{$R_1$} &
%     \colhead{$e$} &
%     \colhead{$i$} &
%     \colhead{$\omega$} &
%     \colhead{$\Omega$} \\
%     \omit &
%     \colhead{(mas)} &
%     \colhead{(mas)}  &
%     \colhead{($\arcdeg$)} &
%     \colhead{(mas)} &
%     \colhead{(mas)} &
%     \colhead{(mas)} &
%     \omit &
%     \colhead{($\arcdeg$)} &
%     \colhead{($\arcdeg$)} &
%     \colhead{($\arcdeg$)} \\
% }
% \tablewidth{0pt}
% \tablecolumns{11}
% \startdata
%   GPI $J$ 20160323 & 1039$\pm$5 & 1380$^{+7}_{-13}$ & 27.1$\pm$0.1 & 7$\pm$2 & -18$\pm$3 & 1032$\pm$6 & 0.020$\pm$0.004 & 76.9$\pm$0.1 & 27.0$\pm$0.1 & -16$^{+11}_{-15}$ \\
% SPHERE $H_2$ & 1031$\pm$1 & 1389$^{+2}_{-1}$ & 26.88$\pm$0.04 & 0.5$\pm$0.6 & -23$\pm$1 & 1032$\pm$1 & 0.046$\pm$0.002 & 76.77$\pm$0.02 & 26.89$\pm$0.04 & -64$^{+2}_{-1}$\\ 
%   GPI $H$ 20160318 & 1032$\pm$3 & 1378$^{+8}_{-18}$ & 26.72$\pm$0.07 & 1$\pm$1 & -13$\pm$2 & 1032$\pm$3 & 0.026$\pm$0.003 & 76.77$\pm$0.09 & 26.73$\pm$0.07 & -63$^{+6}_{-5}$\\
% GPI $K_{1}$ 20150403 & 1035$^{+4}_{-5}$ & 1194$^{+17}_{-13}$ & 26.60$^{+0.08}_{-0.07}$ & 6$\pm$1 & -25$\pm$2 & 1036$^{+4}_{-5}$ & 0.035$\pm$0.003 & 76.41$\pm$0.09 & 26.61$^{+0.08}_{0.07}$ & -46$\pm$5\\
% GPI $K_{2}$ 20150403 & 1036$^{+7}_{-6}$ & 1184$^{+29}_{-17}$ & 26.5$\pm$0.1 & 5$\pm$2 & -24$\pm$3 & 1037$^{+7}_{-6}$ & 0.034$\pm$0.004 & 76.5$\pm$0.1 & 26.5$\pm$0.1 & -49$\pm$7\\
% \enddata
% \tablecomments{The uncertainties listed in this table are the statistical uncertainties from our fits and do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14} and 0.08$\arcdeg$ for SPHERE/IRDIS \citep{maire16}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14} and 0.25 pixels (or 3 mas) for SPHERE/IRDIS \citep{milli17}.}
% \end{deluxetable*}
% \endinput


==> GPI HR 4796A Total Intensity Phase Function arxive version/table4.tex <==
\ProvidesFile{table4.tex}

\begin{deluxetable}{lccc}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Disk Fitting Scattering Parameters\label{tab:mcmc_spf_param}}
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$g_1$} &
    \colhead{$g_2$} &
    \colhead{$\alpha$} \\
}
\tablewidth{0pt}
\tablecolumns{4}
\startdata
   GPI $J$ 20160323 & 0.80$\pm$0.04 & -0.21$\pm 0.03$  & 0.34$\pm$0.03 \\
SPHERE $H_2^{*}$ & 0.90$\pm$0.03 & -0.17$ \pm 0.01$ & 0.32$^{+0.07}_{-0.04}$ \\
   GPI $H$ 20160318 & 0.79$\pm$0.04 & -0.21$\pm$0.01     & 0.30$^{+0.03}_{-0.02}$ \\
   GPI $K_{1}$ 20150403 & 0.94$^{+0.03}_{-0.04}$ & -0.15$\pm$0.01 & 0.5$^{+0.2}_{-0.1}$ \\
   GPI $K_{2}$ 20150403 & 0.94$^{+0.04}_{-0.06}$ & -0.15$\pm$0.02 & 0.5$\pm$0.2 \\
\enddata
\tablenotetext{*}{Derived from a reanalysis of the data as presented in this manuscript and not from \citetalias{milli17}}
\tablecomments{The uncertainties listed in this table are derived from the 16\%, 50\%, and 84\% percentiles of the marginalized posterior distribution for each parameter and for each dataset. They do not include either the uncertainty in the direction of True North or in the position of the star.}
\end{deluxetable}
\endinput

==> table1.tex <==
\ProvidesFile{table1.tex}

\begin{deluxetable*}{llccccccc}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Observations\label{tab:observations}}
\tablewidth{0pt}
\tablehead{
    \colhead{Target} &
    \colhead{UT Date} &
    \colhead{Program} &
    \colhead{Obs. Mode$^{a}$} &
    \colhead{Int.Time} &
    \colhead{No. of} &
    \colhead{Airmass} &
    \colhead{Seeing} &
    \colhead{Field Rot.$^{b}$} \\
    \omit &
    \omit &
    \omit &
    \omit &
    \colhead{(s)} &
    \colhead{Exps.} &
    \omit &
    \colhead{($\arcsec$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{10}
\startdata
HR 4796A & 2016 Mar 23 & GS-2016A-LP-6 & J-Spec$^{c}$ & 29.1 & 59 &  1.02-1.04 & 0.4-0.7 & 48.8 \\ %\hline
HR 4796A & 2016 Mar 18 & GS-2016A-Q-500 & H-Spec & 59.6 & 37 & 1.01-1.02 & 0.5 & 52.7 \\
HR 4796A & 2014 Mar 25 & GS-ENG-GPI-COM & K1-Spec & 59.6 & 20 & 1.01-1.02 & 0.3 & 15.1, 12.6 \\ 
HR 4796A & 2015 Apr 2 & GS-2015A-Q-27 & K1-Spec & 88.7 & 47 & 1.13-1.24, 1.11-1.21 & 0.55 & 8.0, 8.4 \\
HR 4796A & 2015 Apr 3 & GS-2015A-Q-27 & K1-Spec & 88.7 & 46 & 1.01-1.09 & 0.55 & 78.5 \\
HR 4796A & 2015 Apr 3 & GS-2015A-Q-27 & K2-Spec & 88.7 & 23 & 1.02-1.04 & 0.55 & 33.8 \\
%HR 2562 & 2016 Mar 18 & GS-2016A-Q-500 & K2-Spec & 59.6 & 47 & 1.15-1.17 & 0.8 & 25.7 \\
\enddata
\tablecomments{$^{a}$ GPI instrument mode corresponding to choice of filter plus corresponding focal plane and Lyot plane masks and apodizer.\\ $^{b}$ Change in parallactic angle over the course of the observation sequence.\\ $^{c}$ Observation made with nonstandard apodizer (APOD$\_$H$\_$G6205).}
\end{deluxetable*}
\endinput


==> table2.tex <==
\ProvidesFile{table2.tex}

\begin{deluxetable*}{rcccccccccr}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Debris Ring Analyzer Geometric Parameters (Sky-Plane and Disk-Plane)\label{tab:geoparam}} 
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$a'$} &
    \colhead{$e'$} &
    \colhead{$PA'$} &
    \colhead{$\Delta$R.A.$'$} &
    \colhead{$\Delta$Dec.$'$} &
    \colhead{$a$} &
    \colhead{$e$} &
    \colhead{$i$} &
    \colhead{$\omega$} &
    \colhead{$\Omega$} \\
    \omit &
    \colhead{($mas$)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{(mas)} &
    \colhead{(mas)} &
    \colhead{($mas$)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{11}
\startdata
\cutinhead{Mask-and-Interpolate}
   $J$ 20160323 & 1053$\pm$6  & 0.970$\pm$0.001 & 26.2$\pm$0.5   & 6$\pm$4 & -15$\pm$7 & 1053$\pm$6  & 0.02$\pm$0.01 & 75.9$\pm$0.1 & -22$\pm$56 & 26.2$\pm$0.5 \\
   $H$ 20160318 & 1063$\pm$16  &  0.970$\pm$0.002  & 26.5$\pm$0.4 & 0$\pm$8 &  -6$\pm$11 & 1063$\pm$16  &  0.01$\pm$0.02  & 76.5$\pm$0.5 & -61$\pm$180  & 26.5$\pm$0.4 \\
$K_{1}$ 20140325 & 1079$\pm$27  & 0.970$\pm$0.002 & 26.5$\pm$0.4  & 4$\pm$10 & -17$\pm$19 & 1079$\pm$28  & 0.02$\pm$0.02 & 77.0$\pm$0.6 & -44$\pm$62 & 26.5$\pm$0.4 \\ 
$K_{1}$ 20150402 & 1060$\pm$12  & 0.972$\pm$0.002 & 26.6$\pm$0.4  & -1$\pm$6 & -20$\pm$10 & 1061$\pm$12  & 0.04$\pm$0.02 & 76.4$\pm$0.5 & -67$\pm$19 & 26.6$\pm$0.4 \\
$K_{1}$ 20150403 & 1066$\pm$22  & 0.973$\pm$0.002 & 26.5$\pm$0.4  & 8$\pm$8 & -19$\pm$12 & 1066$\pm$22  & 0.02$\pm$0.01 & 76.5$\pm$0.6 & -14$\pm$46 & 26.5$\pm$0.4 \\
$K_{2}$ 20150403 & 1075$\pm$30 &  0.973$\pm$0.003  & 26.5$\pm$0.5 & -6$\pm$9 &  -13$\pm$16 & 1076$\pm$30 & 0.05$\pm$0.02 & 76.7$\pm$0.7 & -79$\pm$22 & 26.5$\pm$0.5 \\
\cutinhead{RDI-NMF}
   $H$ 20160318 & 1069$\pm$18  &  0.970$\pm$0.002  & 26.5$\pm$0.5 & -1$\pm$9 & -14$\pm$14 & 1070$\pm$18  &  0.03$\pm$0.02  & 76.5$\pm$0.5 & -68$\pm$50 & 26.5$\pm$0.5 \\
\cutinhead{RDI-KLIP}
   $H$ 20160318 & 1063$\pm$15  &  0.972$\pm$0.001  & 26.5$\pm$0.4 & 0$\pm$7 & -15$\pm$11 & 1063$\pm$15  &  0.03$\pm$0.01  & 76.3$\pm$0.4 & -65$\pm$30  & 26.5$\pm$0.4 \\
\cutinhead{ADI-KLIP}
   $J$ 20160323 & 1069$\pm$14 & 0.972$\pm$0.002 & 26.5$\pm$0.5 & 2$\pm$7 & -18$\pm$11 & 1069$\pm$14 & 0.03$\pm$0.02 & 76.5$\pm$0.5 & -58$\pm$43 & 26.5$\pm$0.5 \\
   $H$ 20160318 & 1069$\pm$15 & 0.972$\pm$0.002 & 26.5$\pm$0.4 & 0$\pm$7 & -15$\pm$10 & 1069$\pm$15 & 0.03$\pm$0.02 & 76.5$\pm$0.4 & -65$\pm$35 & 26.5$\pm$0.4 \\
$K_{1}$ 20140325 & 1070$\pm$22 & 0.972$\pm$0.002 & 26.4$\pm$0.5 & 1$\pm$9 & -21$\pm$16 & 1070$\pm$22 & 0.04$\pm$0.02 & 76.4$\pm$0.5 & -61$\pm$23 & 26.4$\pm$0.5 \\ 
$K_{1}$ 20150402 & 1077$\pm$16 & 0.973$\pm$0.002 & 26.4$\pm$0.4 & -2$\pm$8 & -21$\pm$13 & 1078$\pm$16 & 0.05$\pm$0.02 & 76.7$\pm$0.5 &  -69$\pm$23 & 26.4$\pm$0.4 \\
$K_{1}$ 20150403 & 1069$\pm$13  & 0.972$\pm$0.002 & 26.4$\pm$0.5  & 1$\pm$7 & -24$\pm$11 & 1069$\pm$13  & 0.04$\pm$0.02 & 76.4$\pm$0.4 & -62$\pm$21 & 26.4$\pm$0.5 \\
$K_{2}$ 20150403 & 1074$\pm$18 &  0.973$\pm$0.002  & 26.5$\pm$0.5 & 0$\pm$8 &  -23$\pm$13 & 1076$\pm$18 & 0.05$\pm$0.02 & 76.6$\pm$0.5 & -65$\pm$24 & 26.5$\pm$0.5 \\
\enddata
\tablecomments{The uncertainties listed in this table are the statistical uncertainties from our fits and do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14}}
%\tablecomments{$^{b}$Change in parallactic angle over the course of the observation sequence}
\end{deluxetable*}

\endinput


==> table3.tex <==
\ProvidesFile{table3.tex}


\begin{deluxetable*}{lccccc}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Disk Fitting Geometry Parameters (Disk Plane)\label{tab:mcmc_geometry_param}}
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$R_1$} &
    \colhead{$e$} &
    \colhead{$i$} &
    \colhead{$\omega$} &
    \colhead{$\Omega$} \\
    \omit &
    \colhead{(mas)} &
    \omit &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} &
    \colhead{($\arcdeg$)} \\
}
\tablewidth{0pt}
\tablecolumns{11}
\startdata
GPI $J$ 20160323 & 1038$\pm$5 & 0.023$\pm$0.004 & 76.9$\pm$0.1 & -28$^{+15}_{-13}$ & 26.8$\pm$0.1 \\
SPHERE $H_2^{*}$ & 1032 $\pm$1 & 0.047$\pm$0.002 & 76.77$\pm$0.03 & -65$\pm$1 & 26.94$\pm$0.04 \\ 
GPI $H$ 20160318 & 1032$\pm$2 & 0.028$\pm$0.003 & 76.81$\pm$0.07 & -64$\pm$4 & 26.7$\pm$0.1\\
GPI $K_{1}$ 20150403 & 1031$\pm$4 & 0.035$^{+0.003}_{-0.002}$ & 76.47$^{+0.07}_{-0.08}$ & -46$\pm$4 & 26.6$\pm$0.6\\
GPI $K_{2}$ 20150403 & 1036$^{+6}_{-7}$ & 0.024$\pm$0.004 & 76.6$\pm$0.1 & -42$^{+12}_{-11}$ & 26.5$\pm$0.1\\
\enddata
\tablenotetext{*}{Derived from a reanalysis of the data as presented in this manuscript and not from \citetalias{milli17}}
\tablecomments{The uncertainties listed in this table are derived from the 16\%, 50\%, and 84\% percentiles of the marginalized posterior distribution for each parameter and for each dataset. They do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14} and 0.08$\arcdeg$ for SPHERE/IRDIS \citep{maire16}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14} and 0.25 pixels (or 3 mas) for SPHERE/IRDIS (\citetalias{milli17}).}
\end{deluxetable*}
\endinput



% \begin{deluxetable*}{rcccccccccc}
% %\tabletypesize{\scriptsize}
% %\rotate
% \tablecaption{Disk Fitting Geometry Parameters\label{tab:mcmcparam}}
% \tablewidth{0pt}
% \tablehead{
%     \omit &
%     \colhead{$R_1'$} &
%     \colhead{$R_2'$} &
%     \colhead{$PA'$} &
%     \colhead{$\Delta$R.A.$'$} &
%     \colhead{$\Delta$Dec.$'$} &
%     \colhead{$R_1$} &
%     \colhead{$e$} &
%     \colhead{$i$} &
%     \colhead{$\omega$} &
%     \colhead{$\Omega$} \\
%     \omit &
%     \colhead{(mas)} &
%     \colhead{(mas)}  &
%     \colhead{($\arcdeg$)} &
%     \colhead{(mas)} &
%     \colhead{(mas)} &
%     \colhead{(mas)} &
%     \omit &
%     \colhead{($\arcdeg$)} &
%     \colhead{($\arcdeg$)} &
%     \colhead{($\arcdeg$)} \\
% }
% \tablewidth{0pt}
% \tablecolumns{11}
% \startdata
%   GPI $J$ 20160323 & 1039$\pm$5 & 1380$^{+7}_{-13}$ & 27.1$\pm$0.1 & 7$\pm$2 & -18$\pm$3 & 1032$\pm$6 & 0.020$\pm$0.004 & 76.9$\pm$0.1 & 27.0$\pm$0.1 & -16$^{+11}_{-15}$ \\
% SPHERE $H_2$ & 1031$\pm$1 & 1389$^{+2}_{-1}$ & 26.88$\pm$0.04 & 0.5$\pm$0.6 & -23$\pm$1 & 1032$\pm$1 & 0.046$\pm$0.002 & 76.77$\pm$0.02 & 26.89$\pm$0.04 & -64$^{+2}_{-1}$\\ 
%   GPI $H$ 20160318 & 1032$\pm$3 & 1378$^{+8}_{-18}$ & 26.72$\pm$0.07 & 1$\pm$1 & -13$\pm$2 & 1032$\pm$3 & 0.026$\pm$0.003 & 76.77$\pm$0.09 & 26.73$\pm$0.07 & -63$^{+6}_{-5}$\\
% GPI $K_{1}$ 20150403 & 1035$^{+4}_{-5}$ & 1194$^{+17}_{-13}$ & 26.60$^{+0.08}_{-0.07}$ & 6$\pm$1 & -25$\pm$2 & 1036$^{+4}_{-5}$ & 0.035$\pm$0.003 & 76.41$\pm$0.09 & 26.61$^{+0.08}_{0.07}$ & -46$\pm$5\\
% GPI $K_{2}$ 20150403 & 1036$^{+7}_{-6}$ & 1184$^{+29}_{-17}$ & 26.5$\pm$0.1 & 5$\pm$2 & -24$\pm$3 & 1037$^{+7}_{-6}$ & 0.034$\pm$0.004 & 76.5$\pm$0.1 & 26.5$\pm$0.1 & -49$\pm$7\\
% \enddata
% \tablecomments{The uncertainties listed in this table are the statistical uncertainties from our fits and do not include either the uncertainty in the direction of True North or in the position of the star. The uncertainty in the measurement of True North is 0.03$\arcdeg$ for GPI \citep{konopacky14} and 0.08$\arcdeg$ for SPHERE/IRDIS \citep{maire16}. The uncertainty in the position of the star is 0.05 pixels (or $\sim$0.7 mas) for GPI \citep{wang14} and 0.25 pixels (or 3 mas) for SPHERE/IRDIS \citep{milli17}.}
% \end{deluxetable*}
% \endinput


==> table4.tex <==
\ProvidesFile{table4.tex}

\begin{deluxetable}{lccc}
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Disk Fitting Scattering Parameters\label{tab:mcmc_spf_param}}
\tablewidth{0pt}
\tablehead{
    \omit &
    \colhead{$g_1$} &
    \colhead{$g_2$} &
    \colhead{$\alpha$} \\
}
\tablewidth{0pt}
\tablecolumns{4}
\startdata
   GPI $J$ 20160323 & 0.80$\pm$0.04 & -0.21$\pm 0.03$  & 0.34$\pm$0.03 \\
SPHERE $H_2^{*}$ & 0.90$\pm$0.03 & -0.17$ \pm 0.01$ & 0.32$^{+0.07}_{-0.04}$ \\
   GPI $H$ 20160318 & 0.79$\pm$0.04 & -0.21$\pm$0.01     & 0.30$^{+0.03}_{-0.02}$ \\
   GPI $K_{1}$ 20150403 & 0.94$^{+0.03}_{-0.04}$ & -0.15$\pm$0.01 & 0.5$^{+0.2}_{-0.1}$ \\
   GPI $K_{2}$ 20150403 & 0.94$^{+0.04}_{-0.06}$ & -0.15$\pm$0.02 & 0.5$\pm$0.2 \\
\enddata
\tablenotetext{*}{Derived from a reanalysis of the data as presented in this manuscript and not from \citetalias{milli17}}
\tablecomments{The uncertainties listed in this table are derived from the 16\%, 50\%, and 84\% percentiles of the marginalized posterior distribution for each parameter and for each dataset. They do not include either the uncertainty in the direction of True North or in the position of the star.}
\end{deluxetable}
\endinput
